Truthful Information Elicitation from Hybrid Crowds

Suppose a decision maker wants to predict weather tomorrow by eliciting and aggregating information from crowd. How can the decision maker incentivize the crowds to report their information truthfully? Many truthful peer prediction mechanisms have been proposed for homogeneous agents, whose types are drawn from the same distribution. However, in many situations, the population is a hybrid crowd of different types of agents with different forms of information, and the decision maker has neither the identity of any individual nor the proportion of each types of agents in the crowd. Ignoring the heterogeneity among the agent may lead to inefficient of biased information, which would in turn lead to suboptimal decisions. In this paper, we propose the first framework for information elicitation from hybrid crowds, and two mechanisms to motivate agents to report their information truthfully. The first mechanism combines two mechanisms via linear transformations and the second is based on mutual information. With two mechanisms, the decision maker can collect high quality information from hybrid crowds, and learns the expertise of agents.

==> May_25_introduction_new.tex <==

\section{Introduction}
Information elicitation is a classical, significant, and ubiquitous problem in our society. Take stock market prediction  for example. Suppose an investor wants to predict whether the stock price of a  company will go either up or down %
by eliciting and aggregating information from the crowd. Often, different types of agents may receive different types of signals. For example, agents with more expertise (referred to as {\em experts} in this paper) may  receive a noisy {\em continuous} signal about the stock  future, for example the probability for the stock price to go up. Agents with less expertise (referred to as {\em non-experts} in this paper) may receive a noisy {\em discrete} signal, i.e.~whether the price will go up or down, but not its likelihood. Moreover, agents may lie about their signals. Suppose the investor does not know whether an agent is an expert or a non-expert or even the percentage of experts in the population, how can she incentivize agents to report their signals truthfully?

In this paper, we focus on designing truthful information elicitation mechanisms from a {\em hybrid crowd} of different types of agents, whose populations are unknown. This happens particularly in crowdsourcing, where the expertise of agents can vary significantly depending on the experiments and it is often hard to estimate the competence level of an agent when the ground truth information is unavailable~\citep{8372965,DellaPenna:2012}. 

One natural and often-used idea is to simply ignore the heterogeneity in the hybrid crowd and apply a peer prediction mechanism that is designed for homogeneous crowd. Unfortunately, this idea does not work well. For example, suppose  a truthful mechanism for continuous signals is applied, e.g.~{the Common Ground mechanism}~\cite{kong2018water}. This incentivizes experts to truthfully report their signals. However, it works poorly for non-experts, because it is unclear even how a sincere non-expert can ``translate'' their continuous signals to discrete reports. Therefore, continuous reports from non-experts can be highly noisy. The problem becomes more complicated when strategic non-experts are involved.

Similarly, suppose we apply a truthful mechanism for discrete signals, for example the {\em Shifted Peer Prediction Mechanism (SPPM)}~\citep{kong2019information}. It works well for non-experts but is problematic for experts, because the experts are forced to report a less informative signal, and it is unclear how strategic experts would behave.

Another natural idea is to let the agents choose their favorite type of signals (i.e.~continuous or discrete) to report. This works well for truthful agents and can lead to more accurate predictions as shown in our MTurk experiments on US presidential election in Section~\ref{sec:mturk}. However, strategic agents may still have incentive to misreport their preferences, and the problem is more challenging than that in the two approaches discussed above, because an agent can now choose to report a signal of any type. For example, a non-expert might be motivated to report a continuous signal for a higher payoff, and an expert might be motivated to report an discrete signal for higher payoff and better privacy.


While there is a large body of literature on truthful information elicitation mechanisms for homogeneous crowds and on estimating agents' competence levels,  the following question is remain open.


{\em  \hfill How can we design   truthful mechanisms to elicit information from hybrid crowd? \hfill}

 



 
\noindent{\bf Our main conceptual contribution} is a framework for information elicitation from hybrid crowd, where  agents have different types of expertise. We also  propose the {\emph{\newtruthfulness}} criterion (Section~\ref{sec:model}), which states that reporting truthful signals is a Bayesian Nash Equilibrium (BNE), and the incentives are  strict unless a misreport leads to the same posterior distribution. This means that any  misreport would not give lead to a strictly higher expected payoff compared to the truthful report, and when the expected payoffs are the same, the misreport contains the same amount of information in  the posterior distribution.\\
{\bf Theoretically, } we focus on a setting with one group experts and two groups of non-experts, and  propose two  mechanisms that satisfy \newtruthfulness{}: the first combines peer prediction mechanisms for homogeneous crowds via linear transformations (Section~\ref{sec:comb}), and the second is  based on mutual information (Section~\ref{sec:mutual}). \\

\noindent{\bf Related Work and Discussions.}  There is a large literature in truthful information elicitation {\em without verification}, a.k.a.~{\em peer prediction}. That is, the ground truth is not available, which in sharp contrast to information elicitation {\em with verification}, in particular the literature in proper scoring rules~\citep{bickel2007some}. Since the seminal work of \citet{miller2005eliciting}, a series of works focus on truth information elicitation from discrete signals~\citep{prelec2004bayesian,radanovic2014incentives,faltings2014incentives,kong2019information}) and continuous signals~\citep{kong2018water}. 
These works focus on proposing truthful mechanisms for homogeneous crowds, while our work considers a hybrid crowd.

Our work is also related to the literature in crowdsourcing on estimating agents' competence, where various statistical algorithms are designed~\citep{Whitehill2009WhoseVS,10.5555/2540128.2540496,10.2307/2346806,10.1007/978-3-642-20161-5_17,BABA20142678,DUAN20145723}. In particular, \citet{10.5555/2540128.2540496} proposed a mechanism where workers report a self-confidence level together with the answer. Practically, crowdsourcing platforms such as Amazon Mechanical Turk and CrowdFlower provide reputation  systems to assess the quality of the crowd worker. However, these  works  do not incentivize workers to provide truthful information. Moreover, these works ask all  agents to report the same type of signals, and therefore fail to distinguish agents of different signal types. On the contrary, our mechanisms incentivize  workers from different crowds  to report truthfully using appropriate user interface corresponding to the types of signals they receive. 

An alternative and plausible approach is to convert the hybrid crowd to a homogeneous crowd by assuming that each agent's signal is  drawn from the set  of all possible signals in the hybrid crowd according to some distributions. However, this approach requires the knowledge of the population of each crowd, which is often unknown in real-life applications for example crowdsourcing tasks, particularly because verifications are not possible.  Our mechanisms do not require such knowledge and is therefore more robust w.r.t.~the uncertainty in the populations of each crowd.




==> composite_old.tex <==
In this section, we introduce our composite elicitation mechanism, which separates three types of agents from each other. Our mechanism combines two single-task information elicitation mechanisms: {\emph {extended common ground mechanism}} (ECGM) and {\emph {shifted peer prediction mechanism}} (SPPM). ECGM takes continuous signals as the input while SPPM takes discrete signal as the input.  Our mechanism combines two mechanisms using a set of linear transformations to achieve the goal of truthfulness.


\subsection{Composite Elicitation Mechanism}\label{subsec: compose}



In \emph{composite elicitation mechanism}, every agent can choose to give a continuous report in $\expset$, a discrete report in $\semiset$, or a discrete report in $\nonset$. %
For an agent $r$, if she chooses to give report in $\expset$, her report is denoted as $\exprep_r$; if she chooses to give report in $\semiset$, her report is denoted as $\semirep_r$; if she chooses to give report in $\nonset$, her report is denoted as $\nonrep_r$. 
 Let $\exprepset$, $\semirepset$ and $\nonrepset$ be the set of agents whose reports are in $\expset$, $\semiset$ and $\nonset$ respectively. The mechanism knows the prior distribution $P$ and the signal distributions of all three types of agents. 

\noindent\textbf{Payment Function} We pay a $\expset$-report agent her ECG mechanism mutual payment with another randomly selected continuous-report agent. (We naturally assume that there are at least 2 reporters of each type.) Formally, if agent $r$ in $\exprepset$ reports a continuous prediction $\exprep_r$, she will be paid $R_{ecg}(\exprep_r, \exprep_j),$ where $j$ is an agent sampled from $\exprepset\setminus\{r\}$ u.a.r.

We pay a $\semiset$-report agent her SPP mechanism mutual payment ($\semiset$ domain) with another randomly selected $\semiset$-report agent, but with a linear transformation corresponding to her own report. 
Formally, for agent $r$ in $\semirepset$ with report $\semirep_r=\semiele_k$, she is paid
\begin{equation*}
    \semiA_k\cdot R_{spp}^{\semiele}(\semirep_r=\semiele_k, \semirep_j)+\semiB_k,
\end{equation*}
where $j$ is an agent sampled from $\semirepset\setminus\{r\}$ u.a.r, and $\semiA, \semiB$ are coefficients of linear transformation. 

We pay a $\nonset$-report agent her SPP mechanism mutual payment ($\nonset$ domain) with another randomly selected $\nonset$-report agent, but with a linear transformation corresponding to her own report. 
Formally, for agent $r$ in $\nonrepset$ with report $\nonrep_r=\nonele_k$, she is paid
\begin{equation*}
    \nonA_k\cdot R_{spp}^{\nonele}(\nonrep_r=\nonele_k, \nonrep_j)+\nonB_k,
\end{equation*}
where $j$ is an agent sampled from $\nonrepset\setminus\{r\}$ u.a.r, and $\nonA, \nonB$ are coefficients of linear transformation. 

The linear transformation coefficients are defined as follows:
for any $k\in[\semisetnum]$, 
\begin{enumerate}
    \item If $\semidist_0^k\neq \semidist_1^k$,
    \begin{equation}
    \label{eq:semiA}
        \semiA_k = \left.\frac{\frac{{\rm d}\exppay_{exp}(\expsig_r, \expsig_r)}{{\rm d}\exppost(\expsig_r)}}{\frac{\partial \semipay_{exp}(\expsig_r,\semiele_k)}{\partial \exppost(\expsig_r)}}\right|_{\exppost(\expsig_r)=\semipost(\semiele_k)}
    \end{equation}
    \begin{equation}
    \label{eq:semiB}
        \semiB_k = \exppay_{non1}(\semiele_k,\expele_r^k) - \semiA_k\cdot \semipay_{non1}(\semiele_k,\semiele_k)
    \end{equation}
    where $\expele_r^k$ satisfies $\exppost(\expele_r^k)=\semipost(\semiele_k)$.
     \item If $\semidist_0^k=\semidist_1^k$, $\semiA_k=\semiB_k=0$.
\end{enumerate}
and for any $k\in[\nonsetnum]$,
\begin{enumerate}
    \item If $\nondist_0^k\neq \nondist_1^k$,
    \begin{equation}
    \label{eq:nonA}
        \nonA_k = \left.\frac{\frac{{\rm d}\exppay_{exp}(\expsig_r, \expsig_r)}{{\rm d}\exppost(\expsig_r)}}{\frac{\partial \nonpay_{exp}(\expsig_r,\nonele_k)}{\partial \exppost(\expsig_r)}}\right|_{\exppost(\expsig_r)=\nonpost(\nonele_k)}
    \end{equation}
    \begin{equation}
    \label{eq:nonB}
        \nonB_k = \exppay_{non2}(\nonele_k,\expele_r^k)) - \nonA_k\cdot \nonpay_{non2}(\nonele_k,\nonele_k)
    \end{equation}
    where $\expele_r^k$ satisfies $\exppost(\expele_r^k)=\nonpost(\nonele_k)$.
     \item If $\nondist_0^k=\nondist_1^k$, $\nonA_k=\nonB_k=0$.
\end{enumerate}
$\exppay, \semipay, \nonpay$ are expected payment of the agents defined as follows:
\footnote{Here $\pdfs[\expsig\mid \expSig_r=\expsig_r]$ is the PDF of $\expSig$ condition on $\expSig_r=\expsig_r$.}
\begin{align}
    \label{eq:CCexp}
    \exppay_{exp}(\expsig_r,\exprep_r)=&\int_{\expset} \pdfs[\expsig\mid \expSig_r=\expsig_r]R_{ecg}(\exprep_r, \expsig){\rm d}\expsig. \\
    \label{eq:SSexp}
    \semipay_{exp}(\expsig_r, \semirep_r)=&\sum_{j=1}^{\semisetnum}\Pr[\semiSig=\semiele_j\mid \expSig_r=\expsig_r]R_{spp}^{\semiele}(\semirep_r, \semiele_j).
\end{align}
\begin{align}
    \label{eq:DDexp}
    \nonpay_{exp}(\expsig_r, \nonrep_r)=&\sum_{j=1}^{\nonsetnum} \Pr[\nonSig=\nonele_j\mid \expSig_r=\expsig_r]R_{spp}^{\nonele}(\nonrep_r, \nonele_j). \\
    \label{eq:CCsemi}
    \exppay_{non1}(\semisig_r,\exprep_r)=&\int_{\expset} \pdfs[\expsig\mid \semiSig_r=\semisig_r]R_{ecg}(\exprep_r, \expsig){\rm d}\expsig. \\
    \label{eq:SSsemi}
    \semipay_{non1}(\semisig_r, \semirep_r)=&\sum_{j=1}^{\semisetnum}\Pr[\semiSig=\semiele_j\mid \semiSig_r=\semisig_r]R_{spp}^{\semiele}(\semirep_r, \semiele_j). \\
    \label{eq:CCnon}
    \exppay_{non2}(\nonsig_r,\exprep_r)=&\int_{\expset} \pdfs[\expsig\mid \nonSig_r=\nonsig_r]R_{ecg}(\exprep_r, \expsig){\rm d}\expsig. \\
    \label{eq:DDnon}
    \nonpay_{non2}(\nonsig_r, \nonrep_r)=&\sum_{j=1}^{\nonsetnum} \Pr[\nonSig=\nonele_j\mid \nonSig_r=\nonsig_r]R_{spp}^{\nonele}(\nonrep_r, \nonele_j). 
\end{align}

$CC_{exp}$ is the expected payment of expert $\AgentR$ when she receives private signal $\expRSig=\expRsig$, and gives continuous report $\expRcardrep$. The other expected payments are defined in the similar way. 
We will give the calculation and analysis of these expected payments in Appendix~\ref{subsec: exppay}. 
(Running Example TBD)

\subsection{Truthfulness of Composite Elicitation Mechanism}

\begin{thm}[Main Theorem]
\label{thm:composite}
The composite elicitation mechanism is truthful. 
\end{thm}

\noindent \textbf{Proof Sketch}
\emph{Truthfulness} can be described as: For any agent, if she believes that all other agents report truthfully in the same form as their private signal, then her expected payment is maximized if she reports truthfully in the same form as her private signal.
Given the expected payment of agents (Equation~\ref{eq:CCexp} to \ref{eq:DDnon}), we can write \emph{truthfulness} as the following two parts:
\begin{enumerate}
    \item \textbf{Interior Truthfulness} If an agent gives a report in the same form as their private signal, her expected payment is maximized when she reports truthfully (i.e. her private signal). 
    \item \textbf{Exterior Truthfulness} If an agent gives a report in other forms, her expected payment will not exceed the payment when she reports truthfully in the same form as their private signal. (Note since their are two other forms, there are also two parts in the exterior truthfulness.) 
\end{enumerate}
The proof will prove the interior truthfulness and two parts of the exterior truthfulness separately for experts and non-experts 1. Non-experts 2 will have the same process of proof as non-experts 1. so the proof is omitted. 

There are two main techniques in the proof. 
The first technique takes advantage of Lemma~\ref{lem:lsr}. It is used to prove several inequality with log function (for example, interior truthfulness of experts). In these cases we rewrite one side of the inequality as the form of one side in Lemma~\ref{lem:lsr} by converting its different parts into different distributions. Then we use Lemma~\ref{lem:lsr} and reach the other side of the inequality. 

The second technique uses derivatives to prove maximum/minimum of certain formula. (for example, in exterior truthfulness of experts towards non-experts 1, we need to prove that $\exppay_{exp}(\expsig_r, \expsig_r) - \semiA_k\semipay_{exp}(\expsig_r,\semiele_k)$ is minimized in some certain $\expsig_r$)
In these cases, we compute the derivative of the formula, and show that the derivative equals to zero in the certain value. Then we compute the second derivative and show it to be strictly monotone. Therefore, the certain value is the unique zero point of the derivative, and therefore the unique minimum/maximum of the formula. 

For some proof like interior truthfulness for non-experts 1, we develop the proof on different cases, and use different techniques in different cases. 

The strictness of interior truthfulness is guaranteed by the strictness of Lemma~\ref{lem:lsr}, which comes from the property of KL-divergence. 


\subsection{Properties of Composite Elicitation Mechanism's Truthful Equilibrium}
In the above section, we show that Composite Elicitation mechanism, for all agents truth-reporting is an equilibrium. While this equilibrium is not a strict one, we can still show that it has many good properties. 
\begin{claim}
For any expert, there are at most $\semisetnum+\nonsetnum$ private signal $\expsig\in \expset$, where the strictness does not hold. 
\end{claim}
This claim shows that the equilibrium is, though not a totally strict one, still very close to the strict BNE. That is, the probability of an expert to be non-strict truthfulness is almost 0. We'll give the proof at the Appendix.
\begin{claim}
For any agent, when she has incentives to report an answer other than her private signal, she will get same payment by answering truthfully and by answering that other signal. 
\end{claim}


==> model_old.tex <==
\noindent\textbf{Ground Truth and Hybrid Crowd.} In this paper we focus on binary ground truth, denoted by $Y\in\{0,1\}$.  The prior distribution over $Y$ is common knowledge, and we let $P=\Pr[Y=1]$. In our model there are three types of agents: the {\em experts}, {\em group 1 non-experts }, and {\em  group 2 non-experts}. 



\noindent\textbf{Private Signals.} Different types of agents receive different types of signals defined. Within each type, each agent's signal is i.i.d.~generated conditioned on the ground truth. The process is illustrated in Figure~\ref{fig:signals} and formally defined as follows.

\noindent $\bullet$ {\bf Experts} receive cardinal signals. Let the experts' signal space $\expset$ be an interval in $\bbR$. We let $\expsig\in\expset$ denote the private signal received by an expert that is represented by a random variable  $\expSig$. Let $f_0$ and $f_1$  denote the PDFs of $S$ given $Y=0$ and $1$,  respectively. 

\noindent $\bullet$ {\bf  Group 1 non-experts} receive ordinal signals. Let $\semiset=\{\semiele_1,\semiele_2,\cdots, \semiele_{\semisetnum}\}$ denote their signal space and let $\semisig\in\semiset$ denote a private signal.  Let $\semiSig$ denote the random variable of a group 1 non-expert's signal, and let  $\semidist_0$ and $\semidist_1$ denote the PMFs of $\semiSig$ given $Y=0$ and $Y=1$, respectively. 



\noindent $\bullet$ {\bf Group 2 non-experts} also receive ordinal signals. Let $\nonset=\{\nonele_1,\nonele_2,\cdots, \nonele_{\nonsetnum}\}$ and let $\nonsig\in\nonset$ denote the signal space and a private signal for a non-expert in group 2, respectively.  Let $\nonSig$ denote the random variable of a group 2 non-expert's signal, and let $\nondist_0$ and $\nondist_1$ denote  the PMFs of  $\nonSig$ given $Y=0$ and $Y=1$, respectively.

\noindent  {\bf Remarks on the notation.} Throughout the paper, a bar over a symbol means that the symbol is defined for group 1 non-experts, for example  $\semiSig$,  $\semidist_0$, and $\semidist_1$. Similarly, a hat over a symbol means that the symbol is defined for group 2 non-experts, for example $\nonSig$,  $\nondist_0$, and $\nondist_1$.

Let us look at an example that corresponds to the experimental setting in Section~\ref{sec:exp}.
\begin{ex}
\label{ex:sig}
We consider about predicting the price of a stock to be low (denoted by $Y=0$) or high ($Y=1$).
The ground truth $y$ is drawn from the prior distribution $P=\Pr[Y=1]=0.5$.  For experts, $\expset=\bbR$ is the expected price of the stock, signal distribution $f_0=N(0, 4)$ (Gaussian distribution with mean 0 and variance 4) and $f_1= N(1, 4)$.

\noindent{Group 1 non-expert $\semiset=\{\text{Very low}, \text{Low}, \text{High}, \text{Very high}\}$. For their signal distributions, we first generate an expert's signal and then check which of the following four interval it falls into:  $\{(-\infty, 0],(0,0.5],(0.5,1],(1,\infty)\}$, and let the interval be the group 1 non-expert's signal.
As a result,  $\semidist_0=[0.50, 0.05,0.05,0.40]$ and $\semidist_1=[0.40,0.05,0.05,0.50]$. }

\noindent{Group 2 non-expert $\nonset=\{\text{Low, High}\}$. Their signals are generated similarly except that we use a more coarse set of two intervals: $\{(-\infty, 0.5],(0.5,\infty)\}$. The result is $\nondist_0=[0.55,0.45]$ and $\nondist_1=[0.45,0.55]$. }




\end{ex}
Our mechanisms and theorems work for a similar setting where there is an expert group and a single non-expert group. The relationships between continuous and discrete signal distributions in this example are not needed for our mechanisms and theorems to hold.

\noindent\textbf{Reports.}
Agents can choose a report in $\Omega = \expset\cup \semiset\cup \nonset$. 
 For any agent $i$,  we denote her report as $\exprep_i,\semirep_i$, and $\nonrep_i$ if she chooses to report in $\expset$, $\semiset$ and $\nonset$, respectively. Let $\exprepset$, $\semirepset$ and $\nonrepset$ denote the set of agents whose reports are in $\expset$, $\semiset$ and $\nonset$ respectively.


\noindent\textbf{Posterior Distributions.} 
Let $\exppost(\expele) \triangleq \Pr[Y=1\mid \expSig=\expele]$ denote the posterior distribution over the ground truth given an expert's signal/report $ \expele$. Similar, let $ \semipost(\semiele)$ (respectively,  $\nonpost(\nonele)$) denote the 
posterior distribution over the ground truth given a group 1 (respectively,  group 2) non-expert's  signal/report
$ \semiele$ (respectively,  $ \nonele$).

\noindent\textbf{Common knowledge.} In this paper, we assume the mechanism, the prior distribution, i.e.~$(1-P,P)$, and the signal distributions, i.e.~$f_i, \semidist_i,  \nondist_i$ for $i\in\{0,1\}$, are common knowledge. Agents' private signals are only known to themselves.


\noindent\textbf{Additional assumptions.}
Throughout the paper, we make the following assumptions on the model. 
The first assumption states that agents' private signals are independent given the ground truth.
\begin{asm}
\label{asm:ci}
Condition on ground truth $Y$, the private signals of all  agents are independent. 
\end{asm}

The second assumption states that agents who receive different private signals have different predictions on others' private signal. 
\begin{asm}
\label{asm:ip}
For any agent $i$ and $j$, the posterior distribution of $j$'s private signal conditional on $i$'s private signal is different for different $i$'s private signal. A formal version can be found in Appendix~\ref{sec:ip}.
\end{asm}
The  two assumption are  standard in the literature, for example, the first can be found in \citep{kong2018water}, and the second can be found in \citep{kong2019information}.

The third assumption has three parts. The first part guarantees that PDFs of experts' signal distributions are strictly positive everywhere. The second and third parts require that the experts' signals are ``richer'' than the group 1 and group 2 non-experts in the sense that for any group 1 (respectively, group 2) non-expert's signal, there exists an expert's signal with the same posterior distribution. 
\begin{asm}
\label{asm:wise}
The experts' signal satisfies the following assumptions:
\begin{enumerate}
    \item for any $\expele \in \expset$, $f(\expele)>0$.
    \item for any $i\in [\semisetnum], \exists \expele \in \expset$, s.t. $\exppost(\expele) = \semipost(\semiele_i)$. 
    \item for any $i\in [\nonsetnum], \exists \expele \in \expset$, s.t. $\exppost(\expele) = \nonpost(\nonele_i)$. 
\end{enumerate}
\end{asm}
We believe the second and third parts of Assumption~\ref{asm:wise}, while being quite technical and primarily used in the proof of the theorem in Section~\ref{sec:comb}, are also very mild, because it does not put any constraints on the distributions---for example it does not require the experts' signals to be more ``concentrated'' around the ground truth.



\textbf{Truthfulness.} One main goal of our mechanism is to elicit truthful information from agents, who can report any signal in $\expset\cup \semiset\cup \nonset$. In this paper, we require the following new notion of truthfulness, called  \textbf{\newtruthfulness}, which is stronger than standard truthfulness and slightly weaker than strict truthfulness. 

\begin{dfn}[\bf \Newtruthfulness]
\label{dfn:truthfulness}
 A mechanism $\mathcal{M}$  is  {\newtruthful} if
 
(1) Truth reporting is a BNE, and (2) Every agent has a strictly higher expected payment for truthful report than another report $s$ if $s$ has a different posterior   distribution over the ground truth. 
\end{dfn}
Clearly, \newtruthfulness{} is stronger than standard truthfulness and weaker than strict truthfulness. We argue that a \newtruthful{} mechanism is not significantly weaker than a strictly truthful mechanism w.r.t.~information elicitation. Notice that a \newtruthful{} mechanism is strictly truthful when  agents' reports are converted to posterior distributions. Therefore, if the posterior distributions of agents' reports contain all information for aggregation, such as in maximum a posteriori (MAP) estimators, then agents have strict incentive to report their truthful information contained in a signal that may or may not be the type of signal she received. 


 




==> preliminary_old.tex <==


\lirong{Qishen and Sikai please prepare this section ASAP so that everyone else will use the same notation.
}



\subsection{Notations}




For any positive integer $n$, we use $[n]$ to denote the set $\{1,2,3,\cdots, n\}$. $\Delta_{\Omega}$ is the set of all distributions over probability space $\Omega$.

{\color{violet} Ao: I summarize the notations as below (I'm not sure on some of them): 
(modified by Qishen)
\begin{itemize}
    \item For expert: private signal $s$ (Use $S$ to represent random variable), prediction of ground truth calculated from private signal $p$, actual continuous report $\hat{p}$, actual discrete report $a$. 
    \item For non-expert: private signal $\tilde{s}$(Use $\tilde{S}$ to represent random variable), prediction of ground truth calculated from private signal $\tilde{p}$, actual continuous report $\hat{p}$, actual discrete report $a$. 
    \qishen{For convenience, I want to change the tilde notations: tilde only exist in non-expert's private signal $\tilde{s}$, and do not use tilde in private prediction $p$, report $\hat{p}$ and $a$. But I haven't examine whether this would cause ambiguity}
    \item Number of experts/non-experts $n_{\text{expert}}$ and $n_{\text{non-expert}}$
    \item Ground truth $Y \in \{0,1\}$ (I would suggest to change this notation because $Y$ is also used as a random variable. PS: changing the notation of random variable $Y$ is also good)(Ground truth is, to some extent, a random variable)
    \item Signal distribution $F_0$ (with PDF $f_0(x)$ and CDF $F_0(x)$) when $Y=0$, and $F_1$ (with PDF $f_1(x)$ and CDF $F_1(x)$). 
    \item The number of discrete signal type: $m$
    \item Thresholds of discrete signal types $t_0=-\infty, t_1,\cdots,t_{m-1}, t_m=\infty$
    \item Discrete signal types $\theta_1,\cdots,\theta_m$
    \item The set of all discrete signal types $\Theta$ %
    \item The set of all thresholds for discrete signal types  $\mathcal{T}$     \item $F_0^k=F_0(t_k)-F_0(t_{k-1})$, and $F_1^k=F_1(t_k)-F_1(t_{k-1})$
    \item (Probably) Some sets of agents (e.g., experts, non-experts, reporting sth and etc.)
    \item $CC_{exp}(p,\hat{p})$ A general expert's expected payment in Extended Common Ground mechanism when she gets private prediction $p$ and reports $\hat{p}$. When $\hat{p}=p$, we use $CC_{exp}(p)$ in abbreviation. 
    \item $DD_{exp}(p,a)$ A general expert's expected payment in SPP mechanism when she gets private prediction $p$ and reports $a$. 
    \item $CC_{non}(\tilde{s}, \hat{p})$ A general non-expert;s expected payment in Extended Common Ground mechanism when she gets private signal $\tilde{s}$ and reports $\hat{p}$.
    \item $DD_{non}(\tilde{s}, a)$ A general non-expert'ss expected payment in SPP mechanism when she gets private signal $\tilde{s}$ and reports $a$. When $a=\tilde{s}$, we use $DD_{non}(\tilde{s})$ in abbreviation. 
\end{itemize}
I would suggest to use ``cal\{\}'' to denote the sets. The upper cases as the random variables and etc.
}

\subsection{KL-Divergence}
\begin{dfn}[Discrete KL-Divergence]
$\Sigma$ is a finite set. The KL-divergence $D_{KL}:\Delta_{\Sigma}\times\Delta_{\Sigma}\mapsto \mathbb{R}$\ao{$\Delta_{\cdot}$ is not defined} is a non-symmetric measure of the difference between distribution $P\in\Delta_{\Sigma}$ and $Q\in \Delta_{\Sigma}$. It is defined as 
$$ D_{KL}(P||Q)=\sum_{\sigma\in\Sigma} P(\sigma)\log\left(\frac{P(\sigma)}{Q(\sigma)}\right),$$
\end{dfn}


\begin{dfn}[Continuous KL-Divergence]
$P$ and $Q$ are distributions of continuous random variables on $\mathbb{R}$. The KL-divergence $D_{KL}:\Delta_{\mathbb{R}}\times \Delta_{\mathbb{R}}\mapsto \mathbb{R}$ is a non-symmetric measure of the difference between $P$ and $Q$. It is defined as 
$$ D_{KL}(P||Q)=\int_{-\infty}^{\infty} p(x)\log\left(\frac{p(x)}{q(x)}\right){\rm d}x, $$
where $p(x)$ and $q(x)$ are the probability density function of $P$ and $Q$. 
\end{dfn}

Both discrete and continuous KL-divergence have the property that for any distribution $P,Q$, $D_{KL}(P||Q)\ge 0$, and the equality holds if and only if $P=Q$. With this property we can prove the following lemma:

\begin{lem}
\label{lem:lsr}
(Discrete Version) $P,Q,R$ are distribution on finite set $\Sigma$. Then we have 
$$ \sum_{\sigma\in\Sigma} P(\sigma)\log\left(\frac{Q(\sigma)}{R(\sigma)}\right) \le \sum_{\sigma\in\Sigma} P(\sigma)\log\left(\frac{P(\sigma)}{R(\sigma)}\right).$$

(Continuous Version) $P,Q,R$ are distributions of continuous random variables on $\mathbb{R}$. Then we have $$ \int_{-\infty}^{\infty} p(x)\log\left(\frac{q(x)}{r(x)}\right){\rm d}x \le \int_{-\infty}^{\infty} p(x)\log\left(\frac{p(x)}{r(x)}\right){\rm d}x.$$

For both version, the equality holds if and only if $P=Q$. 
\end{lem}
The proof of the lemma is in the Appendix. 

\subsection{Shannon Mutual Information}
For two random variables $X$ and $Y$, let $U_{X,Y}$ be the joint distribution of $(X, Y)$ and $V_{X, Y}$ be the product of the marginal distributions of $X$ and $Y$. i.e.
$$U_{X,Y}(X=x,Y=y)=\Pr[X=x,Y=y]$$
$$V_{X,Y}(X=x,Y=y)=\Pr[X=x]\Pr[Y=y]$$
If both $X$ and $Y$ are discrete random variables, we can define Shannon mutual information by discrete KL-divergence.
\begin{dfn}[Discrete-Discrete Shannon Mutual Information]
The Shannon mutual information for two discrete random variables $X$ and $Y$ with finite probability space $\Sigma$ is defined as
\begin{align*}
    MI(X;Y)&=D_{KL}(U_{X,Y}||V_{X,Y})\\
    &=\sum_{x\in\Sigma}\sum_{y\in\Sigma} \Pr[X=x,Y=y]\log\left(\frac{\Pr[X=x,Y=y]}{\Pr[X=x]\Pr[Y=y]}\right)
\end{align*}
\end{dfn}
Similarly, for two continuous random variables, by continuous KL-divergence we have
\begin{dfn}[Continuous-Continuous Shannon Mutual Information]
For two continuous random variable $X$ and $Y$ with probability space $\mathbb{R}$, let $f_X$ and $f_Y$ be the probability density functions of $X$ and $Y$, and let $f_{XY}$ be the probability density function of joint distribution of $(X,Y)$. The Shannon mutual information of $X$ and $Y$ is defined as
\begin{align*}
    MI(X;Y)&=D_{KL}(U_{X,Y}||V_{X,Y})\\
    &=\int_{-\infty}^\infty\int_{-\infty}^\infty f_{XY}(x,y)\log\left(\frac{f_{XY}(x,y)}{f_X(x)f_Y(y)}\right){\rm d}x{\rm d}y
\end{align*}
\end{dfn}
When $X$ is a discrete random variable and $Y$ is a continuous random variable, we can define Shannon mutual information in a similar way.
\begin{dfn}
For discrete random variable $X$ with finite probability space $\Sigma$ and continuous random variable $Y$ with probability space $\mathbb{R}$, let $f_{XY}$ be the probability density function of joint distribution of $(X,Y)$ and $f_Y$ be probability density function of $Y$. The Shannon mutual information of $X$ and $Y$ is defined as
\begin{align*}
    MI(X;Y)=\sum_{x\in\Sigma}\int_{-\infty}^\infty f_{XY}(x,y)\log\left(\frac{f_{XY}(x,y)}{\Pr[X=x]f_y(y)}\right){\rm d}y
\end{align*}
\end{dfn}
For all three types of Shannon mutual information, they satisfy
\begin{enumerate}
    \item \textbf{non-negativity} $MI(X;Y)\ge 0$
    \item \textbf{symmetry} $MI(X;Y)=MI(Y;X)$
\end{enumerate}

\subsection{Pointwise Mutual Information}
For convenience, we define pointwise mutual information $K(X_A=x_A,X_B=x_B)$ for two random variable $X_A$ and $X_B$ as the ratio of $U_{X_A,X_B}(x_A,x_B)$ and $V_{X_A,X_B}(x_A,x_B)$. i.e.
$$K(X_A=x_A,X_B=x_B)=\frac{\Pr[X_A=x_A,X_B=x_B]}{\Pr[X_A=x_A]\Pr[X_B=x_B]}$$
Moreover, if there exists a random variable $Y$ such that $X_A$ and $X_B$ are independent conditioning on $Y$, we have the following formats of pointwise mutual information which are equivalent to the definition.
\begin{claim}
\label{claim:pmi}
When random variable $X_A$ and $X_B$ are independent conditioning on random variable $Y$. i.e.
$$\Pr[X_A,X_B\mid Y]=\Pr[X_A\mid Y]\Pr[X_B\mid Y]$$
the pointwise mutual information $K(X_A=x_A,X_B=x_B)$ has three equivalent formulas
\begin{equation}
\label{pmi:ecg}
    \sum_y\frac{\Pr[Y=y\mid X_A=x_A]\Pr[Y=y\mid X_B=x_B]}{\Pr[Y=y]}
\end{equation}
\begin{equation}
\label{pmi:spp}
    \sum_y\frac{\Pr[X_A=x_A\mid Y=y]\Pr[X_B=x_B\mid Y=y]\Pr[Y=y]}{\Pr[X_A=x_A]\Pr[X_B=x_B]}
\end{equation}
\begin{equation}
\label{pmi:cross}
    \sum_y\frac{\Pr[Y=y\mid X_A=x_A]\Pr[X_B=x_B\mid Y=y]}{\Pr[X_B=x_B]}
\end{equation}
\end{claim}
We will use this property many times in the future. The proof is deferred to the appendix.

\subsection{Proper Scoring Rule}
\label{subsec: ps}
\begin{dfn}[Proper Scoring Rule]
\label{dfn:ps}
A scoring rule $PS:\Omega\times\Delta_{\Omega}\mapsto\mathbb{R}$ takes two coordinates: An element $\omega\in\Omega$, and a distribution $\mathbf{q}\in \Delta_{\Omega}$ and output a real number. A scoring rule is \textit{proper} if when $\omega$ is drawn from $\mathbf{q}$, then the expectation of $PS$ is maximized at $\mathbf{q}$, i.e. for any $\mathbf{p}\in\Delta_{\Omega}$, 
$$ PS(\omega, \mathbf{q})\ge PS(\omega, \mathbf{p}).$$
\end{dfn}
One example of proper scoring rule is log scoring rule, i.e. 
$$L(\omega, \mathbf{q})=\log\left(\mathbf{q}(\omega)\right).$$

